Enhancing Interpretability using Human Similarity Judgements to Prune Word Embeddings

Interpretability methods in NLP aim to provide insights into the semantics underlying specific system architectures. Focusing on word embeddings, we present a supervised-learning method that, for a given domain (e.g., sports, professions), identifies a subset of model features that strongly improve prediction of human similarity judgments. We show this method keeps only 20-40% of the original embeddings, for 8 independent semantic domains, and that it retains different feature sets across domains. We then present two approaches for interpreting the semantics of the retained features. The first obtains the scores of the domain words (co-hyponyms) on the first principal component of the retained embeddings, and extracts terms whose co-occurrence with the co-hyponyms tracks these scores' profile. This analysis reveals that humans differentiate e.g. sports based on how gender-inclusive and international they are. The second approach uses the retained sets as variables in a probing task that predicts values along 65 semantically annotated dimensions for a dataset of 535 words. The features retained for professions are best at predicting cognitive, emotional and social dimensions, whereas features retained for fruits or vegetables best predict the gustation (taste) dimension. We discuss implications for alignment between AI systems and human knowledge.

==> notes.tex <==
spacy pos tags
https://universaldependencies.org/u/pos/


\begin{enumerate}
    \item  \textbf{Feature ranking:} The features within the embedding matrix undergo ranking, where quantification of change with respect to a baseline 2OI is performed. The algorithm is a one-pass forward sequential features selection algorithm. We remove each of the 300 features, compute the RSM from the remaining 299 features, and evaluate the 2OI to the HSJ RSM, quantified by Spearman's rho. The ranking of a feature is defined as the extent to which the removal of the feature increases or decreases the Spearman's correlation between the embeddings matrix and the human similarity matrix. Intuitively, important features are those whose removal produces a lower 2OI than baseline, whereas non-important one are those whose removal does not impact or even improves on the baseline 2OI

    \item \textbf{Insertion of the ranked features:} The ranked features are sequentially added to a new matrix, following their order of importance. From this partial set, an RSM is generated, and the 2OI is computed after each feature insertion. The pruning algorithm selects the set of features that yields the highest 2OI among all the iterations. Word-pair similarity from word embeddings is determined by measuring the cosine distance.
    
\end{enumerate}

Once pruning identifies the subset of features on the train set, only these features are considered for the test-set words and an RSM is computed for the test set, as well as 2OI value for prediction of human similarity judgments.


\begin{algorithm}
 \caption{Pruning: Main algorithm}\label{alg:cap_1}
\begin{algorithmic}\\
\textbf{Inputs}: \\
 \begin{itemize}
    \item $\mathit{SM_{HM}}$: similarity Matrix of human similarity judgments
    \item $\mathit{SM_{DNN}}$: similarity Matrix of similarity estimations derived from the DNN by computing the Pearson's correlation between the embeddings of two images
\end{itemize}\\
\break
\\
\begin{enumerate}
    \item Compute baseline $\mathit{R^{2}(SM_{HM}, SM_{DNN})}$,  using the full set of features.
    \item \textbf{Rank features}
    \begin{itemize}
        \item For each feature:
        \begin{itemize}
            \item Remove the feature from original embeddings, compute reduced similarity matrix $SM_{DNNRED}$.
            \item Calculate difference $D = R^2(SM_{HM}, SM_{DNN}) - R^2(SM_{HM}, SM_{DNNRED})$.
        \end{itemize}
        \item Rank features based on $D$, with higher values indicating great indicating importance.
    \end{itemize}

     \item \textbf{Construct pruned embeddings} \begin{itemize}
        \item Initialize an empty set of features.
        \item Iterate over ranked features in descending order of importance according to $D$
        \begin{itemize}
            \item Reinsert one feature at a time.
            \item Calculate $R^2$ after each feature reinsertion, store values in array $a$.
        \end{itemize}
        \item Determine the maximum value in array $\mathit{a}$. 
        \item The index of the maximum value  delimits the set of features to be included in the pruned embeddings.
     \end{itemize} 
 \end{enumerate}
 \end{algorithmic}
\end{algorithm}






\begin{figure*}[!h]
\includegraphics[width=1.1\textwidth]{images/pruning\_results.jpg}
\centering
\caption{Results of LOOCV pruning using Spearman's correlation as 2OI.}
\label{figure1}
\end{figure*}

\begin{figure*}[!h]
\includegraphics[width=1.1\textwidth]{images/retained\_features.jpg}
\centering
\caption{Average number of features retained after pruning.}
\label{figure2}
\end{figure*}


\begin{table}[tb]
    \centering
    \begin{tabular}{lllll}
    \hline
        \textbf{Category} & \textbf{Hits} & \textbf{Prn} & \textbf{Full} & \textbf{Cmn}\\ \hline
        \textbf{Furniture} & 15968 & 77 & 42 & 35 \\ 
        \textbf{Clothing} & 8615 & 26 & 18 & 5 \\ 
        \textbf{Birds} & 8850 & 27 & 21 & 12 \\ 
        \textbf{Vegetables} & 2888 & 4 & 11 & 2 \\ 
        \textbf{Sports} & 16075 & 114 & 126 & 73\\ 
        \textbf{Vehicles} & 18146 & 29 & 48 & None\\ 
        \textbf{Fruit} & 8263 & 15 & 16 & 2\\ 
        \textbf{Professions} & 25125 & 113 & 161 & 107 \\ \hline
     \end{tabular}
    \caption{For each category, Hits signifies the total number of words in the Category neighborhood. The number of words that significantly correlate with the scores of the category's first principal component when computed from Pruned or Unpruned embeddings.}
    \label{tab:PMI_hits}
\end{table}
